Crossing-Domain Generative Adversarial Networks for Unsupervised Multi-Domain Image-to-Image Translation

State-of-the-art techniques in Generative Adversarial Networks (GANs) have shown remarkable success in image-to-image translation from peer domain X to domain Y using paired image data. However, obtaining abundant paired data is a non-trivial and expensive process in the majority of applications. When there is a need to translate images across n domains, if the training is performed between every two domains, the complexity of the training will increase quadratically. Moreover, training with data from two domains only at a time cannot benefit from data of other domains, which prevents the extraction of more useful features and hinders the progress of this research area. In this work, we propose a general framework for unsupervised image-to-image translation across multiple domains, which can translate images from domain X to any a domain without requiring direct training between the two domains involved in image translation. A byproduct of the framework is the reduction of computing time and computing resources, since it needs less time than training the domains in pairs as is done in state-of-the-art works. Our proposed framework consists of a pair of encoders along with a pair of GANs which learns high-level features across different domains to generate diverse and realistic samples from. Our framework shows competing results on many image-to-image tasks compared with state-of-the-art techniques.

==> background.tex <==
\section{Background}

\begin{comment}
\subsubsection{Variational Autoencoders (VAEs)}

The key of VAEs is to use a learned approximate inference. This is achieved by using a learned approximate posterior $q_{\phi}(z\vert x)=N(\mu, \sigma I)$ whose parameters are given by a neural network referred to as the \textit{encoder}. Thus, we have $z \sim Enc(x)=q(z\vert x)$ and $\hat{x} \sim Dec(z)=p(x\vert z)$. An upper bound on the expected negative log-likelihood of $x$ is derived as objective to optimize the parameters of the networks, given by

\begin{equation}
\mathcal{L} = \mathbb{E}_{q(z\vert \mathbf{x})}[-\log p_{\theta}(x\vert z) + KL[q_{\phi}(z\vert x) \vert \vert p(z)]
\end{equation}

New data samples, not present in the training data, can be generated by first drawing latent samples from the prior $z\sim p(z)$, which is usually a normal distribution, and then drawing data samples from $p_{\theta}(x \vert z)$. However, samples generated by VAEs are often blurry when trained on data from multi-modal distributions.

\end{comment}



\begin{comment}
\subsection{Latent Variable Models}

A \textbf{latent variable model} is a statistical model that relates a set of \textbf{observable variables} to a set of \textbf{latent variables}. The \textbf{observable variables} are assumed to be generated by \textbf{latent variables}, $\textbf{x} \sim p_{\theta}(\textbf{x} \vert \textbf{z})$, where $\textbf{z} \sim p(\textbf{z})$ is the latent variable. $p_{\theta}(\textbf{x} \vert \textbf{z})$ can be represented by a generator (or decoder), $G_{\theta}(\textbf{z})$, with parameters $\theta$. It very useful to get the marginal likelihood $p_{\theta}(\textbf{x})$. However, the marginal likelihood is intractable, which cannot be calculated implicitly. Variational Autoencoders (VAEs) and Generative Adversarial Networks (GANs) are two Deep Generative Models that solve this problem explicitly.

\subsection{Variational Autoencoders}

Variational Autoencoders (VAEs) have emerged as one of the most popular approaches to unsupervised learning of complicated distributions. The key of VAEs is to use a learned approximagte inference that is trained using gradient-based methods. This is achieved by using a learned approximate posterior $q(z\vert x)=N(\mu, \sigma I)$ whose parameters are given by a neural network referred to as the \textit{encoder}.  VAEs are appealing because they are built on top of neural networks, and can be trained with stochastic gradient descent. VAEs have already shown promise in generating many kinds of complicated data.
In Variational Autoencoders (VAEs), a lower bound of the marginal likelihood is derived.

\begin{equation}
\log p_{\mathbf{\theta}}(\mathbf{x}) = \log \int p_{\mathbf{\theta}}(\mathbf{x}\vert \mathbf{z})p(\mathbf{z}) d\mathbf{z} \geq \mathbb{E}_{q_{\mathbf{\eta}}(\mathbf{z}\vert \mathbf{x})}[\log p_{\mathbf{\theta}}(\mathbf{x}\vert \mathbf{z}) - \mathbf{KL}[q_{\mathbf{\eta}}(\mathbf{z}\vert \mathbf{x}) \vert \vert p(\mathbf{z})] = L(\mathbf{\theta}, \mathbf{\eta})
\end{equation}

The variational distribution $q$ is represented as an encoder, which the distribution $p$ is represented as a decoder (or generator). The variational and model parameters are jointly optimized using stochastic gradient descent. 

\subsection{Generative Adversarial Networks}

GANs learn a discriminator that learns to distinguish samples from the true distribution $p_{\ast}(\textbf{x})$ and the model $p_{\theta}(\textbf{x})$. The learning signal that drives the optimization of the model parameters is from the discriminator's ability to distinguish between real and generated data. When the discriminator is unable to distinguish between real and generated data, the training of the model is finished.

The discriminator $D_{\phi}(\mathbf{x}) = p(y=1\vert \mathbf{x})$ that gives the probability that an input $\mathbf{x}$ is from the real distribution, with parameter $\phi$. 

\end{comment}

==> exp2.tex <==
\section{experiment}
\label{exp}

In this section, we conduct experiments by comparing our proposed model with baseline models in terms of image translation quality and efficiency on three datasets.

\subsection{Datasets}

To explore the scalability and effectiveness of our model, we test it on a variety of multi-domain image-to-image translation tasks using the following datasets:

\textbf{Alps Seasons dataset} \cite{2017arXiv171206909A} is collected from images on Flickr. The images are categorized into four seasons based on the provided timestamp of when it was taken. It consists of four categories: \textit{Spring}, \textit{Summer}, \textit{Fall}, and \textit{Winter}. The training data consists of 6053 images of four seasons, while the test data consists of 400 images.

\textbf{Painters dataset} \cite{8237506} includes painting images of four artists \textit{Monet}, \textit{Van Gogh}, \textit{Cezanne}, and \textit{Ukiyo-e}. We use 2851 images as the training set, and 200 images as the test set.

\textbf{CelebA dataset} \cite{Liu:2015:DLF:2919332.2920139} contains ten thousand identities, each of which has twenty images, i.e., two hundred thousand images in total. Each image in CelebA is annotated with 40 face attributes. We resize the initial $178 \times 218$ size images to $256 \times 256$. We randomly select 4000 images as test set and use all remaining images for training data.

We do all the experiments on a Ubuntu system using an Intel i7-6850K, along with a single NVIDIA GTX 1080Ti GPU.

\subsection{Models}
\subsubsection{Baselines Models}

\textbf{CycleGAN} \cite{8237506} This method trains two generators $G: X\rightarrow Y$ and $F: Y\rightarrow X$ in parallel. It not only applies a standard GAN loss respectively for $X$ and $Y$, but applies forward and backward cycle consistency losses which ensure that image $\boldsymbol{x} $ from domain $X$ be translated to image of domain $Y$, which can then be translated back to domain $X$, and vice versa.

\textbf{DiscoGAN} \cite{8237572} This method uses a dual-GAN mechanism, which consists of a primal GAN and a dual GAN. The primal GAN learns to translate images from domain $X$ to domain $Y$, which the dual-GAN learns to invert the task. Images from either domain can be translated and then reconstructed. Thus a reconstruction loss can be used to train the model.

\subsection{Evaluation Metrics}

Evaluating the quality of synthesized images is a challenging problem \cite{NIPS2016_6125}. Recent works have tried using pre-trained semantic classifiers to measure the realism and discriminability of the generated images. The idea is that if the generated images are realistic, classifiers trained on the real images will be able to classify the synthesized images correctly as well. Following \cite{2016arXiv160308511Z, Isola2017ImagetoImageTW, 2016arXiv160305631W}, to evaluate the generative performance of the models quantitatively,  we apply \textit{classification accuracy} on the generated images. For each experiment, we generate enough amount of images of different domains, then we use a pretrained classifier which is trained on the training dataset to classify them to different domains and calculate the classification accuracy.

\subsection{Network Architecture and Implementation Details of Our Model}

For the network architecture, our encoders consists of 3 convolutional layers and 4 basic residual blocks. The generators consisted of 4 basic residual blocks and 3 fractional-strided convolutional layers. The discriminators consisted of stacks of 6 convolutional layers. We use LeakyReLU for nonlinearity. The two encoders share the same parameters on layer 1 and 7, while the two generators share the same parameters on layer 1 and 6, which is the lowest-level layer before the output layer. The details of the networks are given in table \ref{table:architecture}. We evaluate a various of network architectures in the evaluation parts.

The design of the architecture is always a difficult task \cite{2015arXiv151106434R}. To get a proper model architecture, we adopt the architecture of the discriminator from \cite{Isola2017ImagetoImageTW} which has been proved to be proficient in most image-to-image generation tasks. It has 6 convolutional layers. We keep the discriminator architecture fixed and vary the architectures of the encoders and generators. Following the design of the architectures of the generators in \cite{Isola2017ImagetoImageTW}, we use two types of layers, the regular convolutional layers and the basic residual blocks \cite{DBLP:conf/cvpr/HeZRS16}. Since the encoding process is the inverse of the decoding process, we use the same layers for them but put the layers in the inverse orders. The only difference is the first layer of the encoder and the last layer of the generator. We apply $64$ channels for the first layer of the encoders, $3$ channels for the last layer of the generators since the output images have $3$ channels. We gradually change the number of convolutional layers and the number of residual blocks until we get a satisfying architecture. We don't apply \textit{weight sharing} at first. The performance of different architectures are evaluated on the \textit{Painters} dataset and is shown in Fig.~\ref{res_conv}. We can see that when the model has 3 regular convolutional layers and 4 basic residual blocks, the model has the best performance. We keep this architecture fixed for other datasets. 

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{conv_res.png}
\caption{The accuracy on varying number of residual blocks and number of convolutional layers.}
\label{res_conv}
\end{figure}

We then vary the number of weight-sharing layers in the encoders and the generators. We change the number of weight-sharing layers from 1 to 4. Sharing 1 layer in encoders and generators means sharing the first layer for two encoders and the generators (not including the output layer) at the same time. The results are shown in table \ref{tab:share}. We found that sharing 1 layer is enough to have a good performance.

\begin{table}[!t]
\caption{Classification accuracy on number of shared layers in encoders and generators.}
%\renewcommand{\arraystretch}{1.1}
%\small
\centering
\begin{tabular}{ccl}
\toprule
\textbf{\# of shared layers} & \textbf{acc. \% (Painters)} & \textbf{acc. \% (Alps Seasons)} \\
\midrule
0 & 49.75 & 29.95  \\
1 & 52.54 & 33.78 \\
2 & 52.81 & 33.54 \\
3 & 51.13 & 33.06 \\
4 & 51.02 & 32.87 \\
\bottomrule
\end{tabular}
\label{tab:share}
\vspace{-0.2in}
\end{table}

Finally, we fix the network architecture as in Table~\ref{table:architecture}.

\begin{table}[!t]
\caption{Network architecture for the multi-modal unsupervised image-to-image translation experiments. $cxkysz$ denote a Convolution-InstanceNorm-ReLU layer with $x$ filters, kernel size $y$, and stride $z$. $Rm$ denotes a residual block that contains two $3 \times 3$ convolutional layers with the same number of filters on both layer. $un$ denotes a $3 \times 3$ fractional-strided-Convolution-InstanceNorm-ReLU layer with $n$ filters, and stride $\frac{1}{2}$. $n_d$ denotes number of domains. $Y$ and $N$ denote whether the layer is shared or not.}
\small
\centering
\begin{tabular}{cccl}
\toprule
\textbf{Layer} & \textbf{Encoders} & \textbf{Generators} & \textbf{Discriminators}  \\
\midrule
1   &  $c64k7s1 (Y)$ & $R256 (Y)$ & $c64k3s2 (N)$
\\
2 & $c128k3s2(N)$ & $R256 (N)$ & $c128k3s2 (N)$
\\
3  & $c256k3s2 (N)$ & $R256 (N)$ & $c256k3s2 (N)$
\\
4 & $R256 (N)$ & $R256 (N)$ &  $c512k3s2 (N)$
\\
5 & $R256 (N)$ & $u256 (N)$ &  $c1024k3s2 (N)$
\\
6 & $R256 (N)$ & $u128 (Y)$& $c(1+n_d)k2s1 (N)$
\\
7 & $R256 (Y)$& $u3 (N)$ &  
\\
\bottomrule
\end{tabular}

\label{table:architecture}
\vspace{-0.2in}
\end{table}

We use ADAM \cite{2014arXiv1412.6980K} for training, where the training rate is set to 0.0001 and momentums are set to 0.5 and 0.999. Each mini-batch consists of one image from domain $X$ and one image from domain $Y$. Our model has several hyper-parameters. The default values are $\alpha_{0}=10$, $\alpha_1=0.1$, ${\alpha}_2=0.1$, and ${\alpha}_3=10$. The hyper-parameters of the baselines are set to the suggested values by the authors.

\subsection{Quantitative Results}
We evaluate our model on different datasets and compare it with baseline models.
\subsubsection{Comparison on Painters Dataset}

To compare the proposed model with baseline models \textit{Painters} dataset, we first train the state-of-the-art VGG-11 model \cite{2014arXiv1409.1556S} on training data and get a classifier of accuracy 94.5\%. We then score synthesized images by the classification accuracy against the domain labels these photos were synthesized from. We generate around 4000 images for every 5 hours and the classification accuracies are shown in Fig.~\ref{acc_p}.

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{test_acc_pp.png}
\caption{The classification accuracy on \textit{Painters} dataset. The 5 models are the prosed model with \textit{lowest and highest level layers sharing}, \textit{lowest level layers sharing}, \textit{highest level layers sharing}, CycleGAN, and DualGAN.}
\label{acc_p}
\end{figure}

As shown in Fig.~\ref{acc_p}, our model achieves the highest classification accuracy of 52.5\% with training time of 10 hours less than the baseline models.

\subsubsection{Comparison on Alps Seasons Dataset}
We train VGG-11 model on training data of \textit{Alps Seasons} dataset and get a classifier of accuracy 85.5\% trained on the training data. We then classify the generated images by our model and the classification accuracies are shown in Fig.~\ref{acc_a}.

\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{test_acc_a.png}
\caption{The classification accuracy on \textit{Alps Seasons} dataset. The 5 models are the prosed model with \textit{lowest and highest level layers sharing}, \textit{lowest level layers sharing}, \textit{highest level layers sharing}, CycleGAN, and DualGAN.}
\label{acc_a}
\end{figure}

As shown in Fig.~\ref{acc_p}, our model achieves the highest classification accuracy of 33.8\% with training time of 10 hours less than the baseline models.

%\subsubsection{Semi-supervised learning}

%\subsubsection{Training on small datasets}

%\subsubsection{Semantic segmentation metrics}


\subsection{Analysis of the loss function}

We compare the ablations of our full loss. As GAN loss and cycle consistency loss are critical for the training of unsupervised image-to-image translation, we keep these two losses as the baseline model and do the ablation experiments to see the importance of other losses.

\begin{table}
  \caption{Ablation study: classification accuracy of \textit{Painters} and \textit{Alps Seasons} datasets for different losses. The following abbreviations are used: R:reconstruction loss, LCL: latent consistency loss, C: classification loss.}
  \label{tab:abl}
  \begin{tabular}{ccl}
    \toprule
    \textbf{Loss}&\textbf{acc.\% (Painters)}&\textbf{acc. \% (Alps Seasons)}\\
    \midrule
    Baseline & 35.23& 20.81\\
    Baseline + R & 36.86& 21.59\\
    Baseline + LCL & 44.42  & 25.05\\
    Baseline + C & 43.63 & 24.01\\
    Baseline + R + LCL & 45.79 & 27.19 \\
    Baseline + R + C & 44.82 & 26.63 \\
    Baseline + LCL + C & 50.74 & 32.51 \\
    Baseline + R + LCL + C & 52.54 & 33.78 \\
  \bottomrule
\end{tabular}
\end{table}

As shown in Tabel~\ref{tab:abl}, the reconstruction loss is least important with accuracy improvement of about 4.6\% on \textit{Painters} dataset and 3.7\% on \textit{Alps Seasons} dataset. The latent consistency loss brings the model an accuracy improvement of 26.1\% on \textit{Painters} dataset and 20.4\% on \textit{Alps Seasons} dataset. The accuracy is improved by23.8\% on \textit{Painters} dataset and 15.4\% on \textit{Alps Seasons} dataset by the classification loss.

\subsection{Qualitative Results}

Fig.~\ref{painters_r} and Fig.~\ref{ar} show results of the proposed framework on various tasks.


\begin{figure*}[!t]
\begin{minipage}{1\linewidth}
\centering
\subfloat[]{\label{p:m}\includegraphics[scale=.63]{painters_my.png}}
\hspace{2mm}
\subfloat[]{\label{p:c}\includegraphics[scale=.63]{painters_cyc.png}}
\hspace{2mm}
\subfloat[]{\label{p:d}\includegraphics[scale=.63]{painters_du.png}}
\end{minipage}\par
%\begin{minipage}{1\linewidth}
%\centering
%\subfloat[]{\label{res:c}\includegraphics[scale=.38]{3.jpg}}
%\subfloat[]{\label{res:b}\includegraphics[scale=.38]{4.jpg}}
%\end{minipage}\par\medskip
\caption{\textit{Painters} translation results. (a) Images generated by the proposed model. (b) Images generated by CycleGAN. (c) Images generated by DualGAN. Note: The original images are displayed with a dashed square around. The other images are generated according to different domains. The four columns from left to right are \textit{Cezanne}, \textit{Monet}, \textit{Ukiyoe}, and \textit{Vangogh}.}
\label{painters_r}
\vspace{-0.2in}
\end{figure*}






\begin{figure}
\includegraphics[height=3.3in, width=3.3in]{alps_my.png}
\caption{\textit{Alps Seasons} translation results. The original images are displayed with a dashed square around. The other images are generated according to different domains. The four columns from left to right are \textit{Spring}, \textit{Summer}, \textit{Fall}, and \textit{Winter}.}
\label{ar}
\end{figure}


%\subsection{CelebA dataset}
% We construct six domains using the following attributes: black hair, ...


